Learning Optimal Features via Partial Invariance

Learning models that are robust to distribution shifts is a key concern in the context of their real-life applicability. Invariant Risk Minimization (IRM) is a popular framework that aims to learn robust models from multiple environments. The success of IRM requires an important assumption: the underlying causal mechanisms/features remain invariant across environments. When not satisfied, we show that IRM can over-constrain the predictor and to remedy this, we propose a relaxation via $\textit{partial invariance}$. In this work, we theoretically highlight the sub-optimality of IRM and then demonstrate how learning from a partition of training domains can help improve invariant models. Several experiments, conducted both in linear settings as well as with deep neural networks on tasks over both language and image data, allow us to verify our conclusions.

==> tables/apx_DG_with_dist.tex <==

  % Table generated by Excel2LaTeX from sheet 'DG_dist'
%   \begin{table}[!ht]
%     \centering
%       \begin{tabular}{c|cc}
%       \toprule
%           & \multicolumn{2}{c}{Experiment 1: dog(cabinet+bed)} \\
%       \midrule
%       Model & dist from dog(shelf) & Accuracy \\
%       \midrule
%       ERM & 0.17 & 0.771(0.077) \\
%       P-ERM & 0.08 & 0.824(0.007) \\
%       P-ERM & 0.26 & \textbf{0.848(0.106)} \\
%       IRM & 0.17 & 0.767(0.053) \\
%       P-IRM & 0.08 & 0.814(0.104) \\
%       P-IRM & 0.26 & 0.786(0.058) \\
%       \midrule
%           & \multicolumn{2}{c}{Experiment 2:dog(bag+box) } \\
%       \midrule
%           & dist from dog(shelf) & Accuracy \\
%           \midrule
%       ERM & 0.35 & 0.767(0.024) \\
%       P-ERM & 0.52 & 0.533(0.220) \\
%       P-ERM & 0.18 & \textbf{0.914(0.031)} \\
%       IRM & 0.35 & 0.686(0.093) \\
%       P-IRM & 0.52 & 0.562(0.163) \\
%       P-IRM & 0.18 & 0.890(0.064) \\
%       \midrule
%           & \multicolumn{2}{c}{Experiment 3: dog(bench+bike)} \\
%       \midrule
%           & dist from dog(shelf) & Accuracy \\
%           \midrule
%       ERM & 0.54 & 0.709(0.076) \\
%       P-ERM & 0.94 & 0.762(0.083) \\
%       P-ERM & 0.13 & 0.634(0.144) \\
%       IRM & 0.54 & 0.657(0.134) \\
%       P-IRM & 0.94 & \textbf{0.815(0.132)} \\
%       P-IRM & 0.13 & 0.448(0.186) \\
%       \midrule
%           & \multicolumn{2}{c}{Experiment 4: dog(boat+surfboard)} \\
%       \midrule
%           & dist from dog(shelf) & Accuracy \\
%       \midrule
%       ERM & 0.57 & 0.514(0.210) \\
%       P-ERM & 0.12 & 0.800(0.121) \\
%       P-ERM & 1.02 & 0.400(0.164) \\
%       IRM & 0.57 & 0.629(0.187) \\
%       P-IRM & 0.12 & 0.781(0.059) \\
%       P-IRM & 1.02 & 0.495(0.138) \\
%       \bottomrule
%       \end{tabular}%
%          \vspace{6pt}
% \caption{\textbf{Domain generalization in Metashift dataset} Results of partial invariance following the experiments in the original paper of Metashift. The testing }
%     \label{tab:apx_dg_with_dist}%
%   \end{table}%
  % Table generated by Excel2LaTeX from sheet 'DG_dist'
  \begin{table*}[!ht]
    \centering
      \begin{tabular}{c|cccc}
      \toprule
      \multicolumn{1}{c}{} & \multicolumn{1}{p{8.165em}}{Experiment 1: dog(cabinet+bed)} & \multicolumn{1}{p{9.25em}}{Experiment 2:dog(bag+box) } & \multicolumn{1}{p{7.25em}}{Experiment 3: dog(bench+bike)} & \multicolumn{1}{p{9.085em}}{Experiment 4: dog(boat+surfboard)} \\
      \midrule
          & dist = 0.17 & dist = 0.35 & dist = 0.54 & dist = 0.57 \\
      ERM & 0.771(0.077) & 0.767(0.024) & 0.709(0.076) & 0.514(0.210) \\
      P-ERM & \textbf{0.848(0.106)} & \textbf{0.914(0.031)} & 0.762(0.083) & \textbf{0.800(0.121)} \\
      IRM & 0.767(0.053) & 0.686(0.093) & 0.657(0.134) & 0.629(0.187) \\
      P-IRM & 0.814(0.104) & 0.890(0.064) & \textbf{0.815(0.132)} & 0.781(0.059) \\
      \midrule
      \multicolumn{1}{c}{\textcolor[rgb]{ .129,  .129,  .129}{}} & \multicolumn{1}{p{8.165em}}{Experiment 1: truck(cone+fence)} & \multicolumn{1}{p{9.25em}}{Experiment 2:truck(bike+mirror) } & \multicolumn{1}{p{7.25em}}{Experiment 3: truck(flag+tower)} & \multicolumn{1}{p{9.085em}}{Experiment 4: truck(traffic light+dog)} \\
      \midrule
      \textcolor[rgb]{ .129,  .129,  .129}{} & \textcolor[rgb]{ .129,  .129,  .129}{dist = 0.09} & \textcolor[rgb]{ .129,  .129,  .129}{dist = 0.14} & \textcolor[rgb]{ .129,  .129,  .129}{dist = 0.26} & \textcolor[rgb]{ .129,  .129,  .129}{dist = 0.31} \\
      ERM & 0.889(0.044) & \textbf{0.961(0.028)} & 0.817(0.085) & 0.822(0.172) \\
      P-ERM & \textbf{0.944(0.008)} & 0.922(0.069) & 0.667(0.082) & 0.861(0.102) \\
      IRM & 0.872(0.091) & 0.945(0.021) & \textbf{0.906(0.044)} & 0.800(0.141) \\
      P-IRM & 0.911(0.126) & 0.939(0.055) & 0.778(0.039) & \textbf{0.967(0.013)} \\
      \bottomrule
      \end{tabular}%
             \vspace{6pt}
\caption{\textbf{Domain generalization in Metashift dataset} Results of partial invariance following the experiments in the original paper of Metashift. The first set of experiments are for cat and dog images with testing on dog(shelf). The second set is trained on truck and bus images and tested on truck(airplane) images.}
    \label{tab:apx_dg_with_dist}%
  \end{table*}%




==> tables/apx_metashift_dg_results.tex <==
  % Table generated by Excel2LaTeX from sheet 'combined_G0_G4'
%   \begin{table}[!ht]
%     \centering
    
%       \begin{tabular}{c|cccc}
%       \toprule
%           & fence & shelf & floor & woman \\
%       \midrule
%       Model & \textit{$s = 5.7$} & \textit{$s = 9.3$} & \textit{$s = 17.8$} & \textit{$s = 27.4$} \\
%       \midrule
%       ERM & 0.730(0.037) & 0.727(0.022) & 0.724(0.035) & 0.747(0.036) \\
%       IRM & 0.729(0.032) & 0.742(0.036) & 0.723(0.025) & 0.749(0.037) \\
%       P-IRM (d=0) & 0.721(0.041) & \textbf{0.786(0.021)} & \textbf{0.741(0.035)} & 0.775(0.031) \\
%       P-IRM (d=4) & 0.713(0.038) & 0.776(0.060) & 0.736(0.039) & 0.769(0.036) \\
%       P-IRM (d=6) & 0.720(0.023) & 0.808(0.039) & 0.739(0.010) & 0.787(0.026) \\
%       P-IRM (d=10) & \textbf{0.737(0.029)} & 0.785(0.025) & 0.727(0.025) & \textbf{0.802(0.032)} \\
%       \bottomrule
%       \end{tabular}%
%     \vspace{6pt}
%     \caption{\textbf{Domain Generalization in Metashift dataset}: Contexts selected for testing are not seen during training. Similarity $s$ is quantified based on the maximum flow of weights between a context node and the training set. P-IRM model is selected based on  each testing node similarity with a partition $P_k$}
%     \label{tab:apx_metashift_dg_results}%
%   \end{table}%
  % Table generated by Excel2LaTeX from sheet 'G_0_erm_ibirm'
    % Table generated by Excel2LaTeX from sheet 'G_0_erm_ibirm'
  \begin{table*}[!ht]
    \centering
      \begin{tabular}{ccccc}
      \toprule
          & fence & shelf & floor & woman \\
      \midrule
      Model & s = 5.7 & s = 9.3 & s = 17.8 & s = 27.4 \\
      \midrule
      ERM & 0.730(0.037) & 0.727(0.022) & 0.724(0.035) & 0.747(0.036) \\
      P-ERM ($d=0$) & \multicolumn{1}{l}{0.714(0.020)} & \multicolumn{1}{l}{\textbf{0.821(0.035)}} & \multicolumn{1}{l}{\textbf{0.777(0.030)}} & \multicolumn{1}{l}{0.763(0.037)} \\
      P-ERM ($d=4$) & 0.714(0.020) & 0.821(0.035) & 0.777(0.030) & 0.763(0.037) \\
      P-ERM ($d=6$) & 0.716(0.044) & 0.804(0.032) & 0.751(0.025) & \textbf{0.778(0.055)} \\
      P-ERM ($d=10$) & 0.733(0.035) & 0.795(0.033) & 0.744(0.030) & 0.791(0.032) \\
      \midrule
      IRM & 0.729(0.032) & 0.742(0.036) & 0.723(0.025) & 0.749(0.037) \\
      P-IRM ($d=0$) & \multicolumn{1}{l}{0.721(0.041)} & \multicolumn{1}{l}{0.786(0.021)} & \multicolumn{1}{l}{0.741(0.035)} & \multicolumn{1}{l}{0.775(0.031)} \\
      P-IRM ($d=4$) & 0.713(0.038) & 0.776(0.060) & 0.736(0.039) & 0.769(0.036) \\
      P-IRM ($d=6$) & 0.720(0.023) & 0.808(0.039) & 0.739(0.010) & 0.787(0.026) \\
      P-IRM ($d=10$) & 0.737(0.029) & 0.785(0.025) & 0.727(0.025) & 0.802(0.032) \\
      \midrule
      IB\_IRM & 0.729(0.032) & 0.742(0.036) & 0.723(0.025) & 0.749(0.037) \\
      P-IB\_IRM ($d=0$) & \multicolumn{1}{l}{0.713(0.038)} & \multicolumn{1}{l}{0.776(0.060)} & \multicolumn{1}{l}{0.736(0.039)} & \multicolumn{1}{l}{0.769(0.036)} \\
      P-IB\_IRM ($d=4$) & 0.713(0.038) & 0.776(0.060) & 0.736(0.039) & 0.769(0.036) \\
      P-IB\_IRM ($d=6$) & \textbf{0.787(0.026)} & 0.808(0.039) & 0.739(0.010) & 0.720(0.023) \\
      P-IB\_IRM ($d=10$) & 0.737(0.029) & 0.785(0.025) & 0.727(0.025) & 0.802(0.032) \\
      \bottomrule
      \end{tabular}%
    \vspace{6pt}
    \caption{\textbf{Domain Generalization in Metashift dataset}: Contexts selected for testing are not seen during training. Similarity $s$ is quantified based on the maximum flow of weights between a context node and the training set. P-IRM model is selected based on  each testing node similarity with a partition $P_k$}
    \label{tab:apx_metashift_dg_results}%
  \end{table*}%


==> tables/apx_params_metashift.tex <==
  % Table generated by Excel2LaTeX from sheet 'params table Metashift'
  \begin{table*}[!ht]
    \centering
      \begin{tabular}{ll}
      \toprule
      Hyperparameter & Values \\
      \midrule
      Number of epochs & 80 \\
      Batch size & 8 \\
      Learning rate & $10^{-5}$ \\
      Optimizer & Adam \\
      IRM Penalty & 100 \\
      IRM Annealing Iterations & 100 \\
      \bottomrule
      \end{tabular}%
    \vspace{6pt}
    \caption{Hyperparameters for experiments on the Metashift dataset, following choices in \cite{ishaanGP2020, liang2022metashift}}
    \label{tab:apx_params_metashift}%
  \end{table*}%


==> tables/housing_results.tex <==
  % Table generated by Excel2LaTeX from sheet 'Sheet1'
  % Table generated by Excel2LaTeX from sheet 'Sheet1'



==> tables/language_results.tex <==

  
    % Table generated by Excel2LaTeX from sheet 'scierc_best_models_erm_irm_ibir'
  \begin{table*}[!ht]
    \centering
      \begin{tabular}{c|ccc}
      Model & Number of envs & Training Years & Testing accuracy (2010-2016) \\
      \midrule
      ERM & 4   & 1980-2009 & 0.800 (0.012) \\
      IRM & 4   & 1980-2009 & 0.795 (0.005) \\
      P-IRM (paritioned) & 3   & 1990-2009 & 0.795 (0.017) \\
      P-IRM (paritioned) & 2   & 2000-2009 & 0.807 (0.005) \\
      P-IRM (conditioned) & 3   & 1990-2009 & \textbf{0.812 (0.008)} \\
      P-IRM (conditioned) & 2   & 2000-2009 & 0.807 (0.015) \\
      \bottomrule
      \end{tabular}%
   \vspace{6pt}
    \caption{\textbf{Language shifts}: The effect of partitioning on the performance on texts belonging to years from 2010 to 2017. Complete results in Appendix}
    \label{tab:language_results}
  \end{table*}%



==> tables/meta_shift_domain_generalization.tex <==

%   \begin{table}[!ht]
%     \centering
%       \begin{tabular}{c|cccc}
%       \toprule
%       \multicolumn{1}{c}{} & fence & shelf & floor & woman \\
%       \midrule
%           & \textit{$s = 5.7$} & \textit{$s = 9.3$} & \textit{$s = 17.8$} & \textit{$s = 27.4$} \\
%       \midrule
%       IRM & \textbf{0.730(0.02)} & 0.728(0.04) & 0.753(0.02) & \textbf{0.744(0.02)} \\
%       P-IRM (d=0) & 0.727(0.05) & \textbf{0.803(0.03)} & \textbf{0.780(0.02)} & 0.736(0.04) \\
%       \midrule
%       IRM & 0.730(0.02) & 0.728(0.04) & 0.753(0.02) & 0.744(0.02) \\
%       P-IRM (d=4) & \textbf{0.758(0.06)} & \textbf{0.808(0.04)} & \textbf{0.783(0.01)} & \textbf{0.772(0.02)} \\
%       \bottomrule
%       \end{tabular}%
%      \vspace{6pt}
    
%     \caption{\textbf{Domain Generalization in Metashift dataset}: Testing communities are not seen during training. Similarity $s$ is quantified based on the maximum flow of weights between a community and $P_k$.}
%     \label{tab:metashift_domain_genaralization}
%   \end{table}%
  % Table generated by Excel2LaTeX from sheet 'G_0_erm_ibirm'
  \begin{table*}[!ht]
    \centering
      \begin{tabular}{lllll}
      \toprule
          & fence & shelf & floor & woman \\
      \midrule
      Model & s = 5.7 & s = 9.3 & s = 17.8 & s = 27.4 \\
      \midrule
      ERM & \textbf{0.730(0.037)} & 0.727(0.022) & 0.724(0.035) & 0.747(0.036) \\
      P-ERM & 0.714(0.020) & \textbf{0.821(0.035)} & \textbf{0.777(0.030)} & 0.763(0.037) \\
      \midrule
      IRM & 0.729(0.032) & 0.742(0.036) & 0.723(0.025) & 0.749(0.037) \\
      P-IRM & 0.721(0.041) & 0.786(0.021) & 0.741(0.035) & \textbf{0.775(0.031)} \\
      \midrule
      IB\_IRM & 0.729(0.032) & 0.742(0.036) & 0.723(0.025) & 0.749(0.037) \\
      P-IB\_IRM & 0.713(0.038) & 0.776(0.060) & 0.736(0.039) & 0.769(0.036) \\
      \bottomrule
      \end{tabular}%
   \vspace{6pt}
    \caption{\textbf{Domain Generalization in Metashift dataset}: Testing communities are not seen during training. Similarity $s$ is quantified based on the maximum flow of weights between a community and $P_k$. Complete results in Appendix}
    \label{tab:metashift_domain_genaralization}
  \end{table*}%


==> tables/metashift_results_d_4.tex <==
  % Table generated by Excel2LaTeX from sheet '16-05-ii'
   % Table generated by Excel2LaTeX from sheet '16-05-ii'
  \begin{table}[!ht]
    \centering
      \begin{tabular}{c|cc|cc|cc}
      \toprule
          & \multicolumn{2}{c|}{Avg. Acc} & \multicolumn{2}{c|}{Avg. Minority Group Acc} & \multicolumn{2}{c}{Worst Group Acc.} \\
          \midrule
      p   & IRM & P-IRM & IRM & P-IRM & IRM & P-IRM \\
      \midrule
      50  & \textbf{0.847(0.010)} & 0.842(0.011) & 0.860(0.025) & \textbf{0.862(0.019)} & \textbf{0.817(0.024)} & 0.813(0.026) \\
      25  & 0.816(0.022) & \textbf{0.825(0.008)} & 0.818(0.024) & \textbf{0.828(0.012)} & 0.777(0.056) & \textbf{0.797(0.012)} \\
      12  & 0.827(0.009) & \textbf{0.853(0.019)} & 0.822(0.018) & \textbf{0.860(0.033)} & 0.807(0.017) & \textbf{0.830(0.014)} \\
      6   & 0.842(0.028) & \textbf{0.848(0.020)} & 0.847(0.031) & \textbf{0.850(0.014)} & 0.823(0.041) & \textbf{0.830(0.045)} \\
      1   & 0.778(0.059) & \textbf{0.832(0.014)} & 0.787(0.070) & \textbf{0.855(0.025)} & 0.813(0.045) & \textbf{0.817(0.012)} \\
      \bottomrule
      \end{tabular}%

    \vspace{6pt}
    \caption{\textbf{Subpopulation shifts in MetaShift dataset}: Results under the setting of 6 duplicated communities in each environment with \textit{\textbf{p}} indicating the proportion of the minority group to the majority in each environment.}
  \label{tab:metashift_results_d_6}%
  \end{table}%



==> tables/metashift_results_p_1.tex <==
% Table generated by Excel2LaTeX from sheet 'snapshot of results (equal val)'
  % Table generated by Excel2LaTeX from sheet 'Sheet1'
%   \begin{table}[!ht]
%     \centering
%       \begin{tabular}{c|cccc}
%       \toprule
%       \multicolumn{1}{c}{} & \multicolumn{2}{c}{Avg. Acc} & \multicolumn{2}{c}{Avg. Minority Group Acc} \\
%       dup & IRM & P-IRM & IRM & P-IRM \\
%       \midrule
%       0   & 0.797(0.03) & \textbf{0.835(0.02)} & 0.785(0.06) & \textbf{0.825(0.01)} \\
% \cmidrule{2-5}      4   & 0.811(0.01) & \textbf{0.823(0.02)} & 0.793(0.01) & \textbf{0.820(0.05)} \\
% \cmidrule{2-5}      6   & \textbf{0.838(0.01)} & 0.834(0.01) & \textbf{0.825(0.01)} & 0.814(0.02) \\
% \cmidrule{2-5}      10  & \textbf{0.844(0.01)} & 0.826(0.03) & 0.815(0.02) & \textbf{0.828(0.03)} \\
%       \bottomrule
%       \end{tabular}%
%     \vspace{6pt}
%     \caption{\textbf{Subpopulation shifts in MetaShift dataset}: Results under the setting where minority group size is 1\% of the majority group size. The number of duplicated communities in each environment is contributing to the P-IRM performance}
%   \label{tab:metashift_results_p_1}%
% \end{table}%

  % Table generated by Excel2LaTeX from sheet '16-05-ii'
  \begin{table}[!ht]
    \centering
      \begin{tabular}{c|llll}
      \toprule
          & \multicolumn{2}{c}{Avg. Acc} & \multicolumn{2}{c}{Avg. Worst Group Acc} \\
      \midrule
      d   & \multicolumn{1}{c}{IRM} & \multicolumn{1}{c}{P-IRM} & \multicolumn{1}{c}{IRM} & \multicolumn{1}{c}{P-IRM} \\
      \midrule
      0   & 0.837(0.008) & \textbf{0.838(0.015)} & \textbf{0.862(0.009)} & 0.848(0.021) \\
      4   & \textbf{0.811(0.014)} & 0.808(0.012) & 0.792(0.020) & 0.792(0.040) \\
      6   & 0.778(0.059) & \textbf{0.832(0.014)} & 0.787(0.070) & \textbf{0.855(0.025)} \\
      10  & 0.850(0.013) & \textbf{0.853(0.013)} & 0.833(0.012) & \textbf{0.842(0.021)} \\
      \bottomrule
      \end{tabular}%
    \vspace{6pt}
    \caption{\textbf{Subpopulation shifts in MetaShift dataset}: Results under the setting where minority group size is 1\% of the majority group size. The number of duplicated communities in each environment is contributing to the P-IRM performance}
  \label{tab:metashift_results_p_1}%
  \end{table}%


==> tables/metashift_subpopulation_results_all.tex <==
%   % Table generated by Excel2LaTeX from sheet 'irm_pirm_subpopulationshifts_re'
%   \begin{table}[!ht]
%     \centering
%       \begin{tabular}{cccccc}
%       \toprule
%       \multicolumn{6}{c}{Avg. Accuracy} \\
%       \midrule
%       Model & 50\% & 25\% & 12\% & 6\% & 1\% \\
%       \midrule
%       ERM & 0.845(0.019) & 0.850(0.034) & \textbf{0.858(0.020)} & 0.852(0.024) & 0.831(0.032) \\
%       IRM & 0.844(0.042) & 0.857(0.019) & 0.853(0.019) & 0.850(0.039) & 0.823(0.029) \\
%       P-IRM ($d=0$) & 0.854(0.013) & 0.863(0.018) & 0.851(0.014) & 0.843(0.014) & 0.828(0.011) \\
%       P-IRM ($d=4$) & 0.863(0.016) & \textbf{0.869(0.012)} & 0.852(0.025) & 0.858(0.013) & 0.853(0.021) \\
%       P-IRM ($d=6$) & \textbf{0.866(0.013)} & 0.865(0.015) & 0.843(0.030) & \textbf{0.860(0.023)} & \textbf{0.860(0.013)} \\
%       P-IRM ($d=10$) & 0.865(0.021) & 0.855(0.023) & 0.854(0.024) & 0.852(0.013) & 0.856(0.024) \\
%       \midrule
%       \multicolumn{6}{c}{Avg. Minority Group Accuracy} \\
%       \midrule
%       ERM & 0.864(0.022) & 0.862(0.039) & \textbf{0.877(0.031)} & \textbf{0.868(0.030)} & 0.830(0.032) \\
%       IRM & 0.860(0.048) & 0.874(0.026) & 0.868(0.025) & 0.864(0.047) & 0.826(0.033) \\
%       P-IRM ($d=0$) & 0.866(0.015) & 0.871(0.020) & 0.859(0.023) & 0.845(0.021) & 0.832(0.018) \\
%       P-IRM ($d=4$) & 0.873(0.019) & 0.880(0.014) & 0.859(0.027) & 0.864(0.016) & 0.865(0.020) \\
%       P-IRM ($d=6$) & 0.880(0.023) & \textbf{0.882(0.018)} & 0.850(0.041) & 0.866(0.027) & \textbf{0.871(0.021)} \\
%       P-IRM ($d=10$) & \textbf{0.888(0.020)} & 0.857(0.030) & 0.867(0.021) & 0.866(0.014) & 0.860(0.032) \\
%       \midrule
%       \multicolumn{6}{c}{Worst Group Accuracy} \\
%       \midrule
%       ERM & 0.825(0.032) & 0.835(0.057) & 0.830(0.036) & 0.829(0.034) & 0.805(0.031) \\
%       IRM & 0.826(0.064) & 0.829(0.047) & 0.811(0.028) & 0.826(0.040) & 0.797(0.034) \\
%       P-IRM ($d=0$) & 0.820(0.041) & 0.834(0.034) & 0.834(0.046) & 0.821(0.025) & 0.819(0.032) \\
%       P-IRM ($d=4$) & 0.838(0.020) & \textbf{0.853(0.033)} & 0.838(0.033) & \textbf{0.840(0.020)} & 0.832(0.043) \\
%       P-IRM ($d=6$) & \textbf{0.848(0.027)} & 0.835(0.038) & 0.829(0.032) & 0.852(0.027) & \textbf{0.849(0.012)} \\
%       P-IRM ($d=10$) & 0.836(0.039) & 0.842(0.037) & \textbf{0.840(0.043)} & 0.821(0.035) & 0.848(0.036) \\
%       \bottomrule
%       \end{tabular}%
%     \vspace{6pt}
%     \captionsetup{width=1\textwidth}
%     \caption{\textbf{Subpopulation shifts in MetaShift dataset}: In subpopulation shifts, the testing environments are observed during training, but differ in proportions. Results of models under the existence of minority environments in the training data. Here, the percentages of minority environments to the majority environments are $p \in \{50, 25, 12, 6, 1\}$. For P-IRM models, \textbf{\textit{d}} indicates the number of imported nodes at each partition. The lower the percentage the more challenging the training setting is}    \label{tab:apx_subpopulation_all}%
%   \end{table}%

  % Table generated by Excel2LaTeX from sheet 'sub_all'
  \begin{table*}[!ht]
    \centering
      \begin{tabular}{clllll}
      \toprule
      \multicolumn{6}{c}{Avg. Accuracy} \\
      \midrule
      Model & \multicolumn{1}{c}{50\%} & \multicolumn{1}{c}{25\%} & \multicolumn{1}{c}{12\%} & \multicolumn{1}{c}{6\%} & \multicolumn{1}{c}{1\%} \\
      \midrule
      ERM & \multicolumn{1}{c}{0.845(0.019)} & \multicolumn{1}{c}{0.850(0.034)} & \multicolumn{1}{c}{0.858(0.020)} & \multicolumn{1}{c}{0.852(0.024)} & \multicolumn{1}{c}{0.831(0.032)} \\
      P-ERM ($d=0$) & 0.864(0.019) & 0.866(0.010) & \textbf{0.870(0.014)} & 0.860(0.018) & 0.843(0.009) \\
      P-ERM ($d=4$) & \multicolumn{1}{c}{0.864(0.014)} & \multicolumn{1}{c}{\textbf{0.873(0.010)}} & \multicolumn{1}{c}{0.870(0.016)} & \multicolumn{1}{c}{0.853(0.022)} & \multicolumn{1}{c}{0.857(0.023)} \\
      P-ERM ($d=6$) & \multicolumn{1}{c}{\textbf{0.870(0.016)}} & \multicolumn{1}{c}{0.862(0.022)} & \multicolumn{1}{c}{0.866(0.011)} & \multicolumn{1}{c}{0.857(0.020)} & \multicolumn{1}{c}{\textbf{0.868(0.012)}} \\
      P-ERM ($d=10$) & 0.857(0.021) & 0.844(0.042) & 0.854(0.013) & \textbf{0.863(0.016)} & \multicolumn{1}{c}{0.863(0.022)} \\
      \midrule
      IRM & \multicolumn{1}{c}{0.844(0.042)} & \multicolumn{1}{c}{0.857(0.019)} & \multicolumn{1}{c}{0.853(0.019)} & \multicolumn{1}{c}{0.850(0.039)} & \multicolumn{1}{c}{0.823(0.029)} \\
      P-IRM ($d=0$) & \multicolumn{1}{c}{0.854(0.013)} & \multicolumn{1}{c}{\underline{0.863(0.018)}} & \multicolumn{1}{c}{0.851(0.014)} & \multicolumn{1}{c}{0.843(0.014)} & \multicolumn{1}{c}{0.828(0.011)} \\
      P-IRM ($d=4$) & \multicolumn{1}{c}{0.863(0.016)} & \multicolumn{1}{c}{0.869(0.012)} & \multicolumn{1}{c}{0.852(0.025)} & \multicolumn{1}{c}{0.858(0.013)} & \multicolumn{1}{c}{0.853(0.021)} \\
      P-IRM ($d=6$) & \multicolumn{1}{c}{\underline{0.866(0.013)}} & \multicolumn{1}{c}{0.865(0.015)} & \multicolumn{1}{c}{0.843(0.030)} & \multicolumn{1}{c}{\underline{0.860(0.023)}} & \multicolumn{1}{c}{\underline{0.860(0.013)}} \\
      P-IRM ($d=10$) & \multicolumn{1}{c}{0.865(0.021)} & \multicolumn{1}{c}{0.855(0.023)} & \multicolumn{1}{c}{\underline{0.854(0.024)}} & \multicolumn{1}{c}{0.852(0.013)} & \multicolumn{1}{c}{0.856(0.024)} \\
      \midrule
      IB\_IRM & 0.844(0.042) & 0.857(0.019) & 0.853(0.019) & 0.850(0.039) & 0.823(0.029) \\
      P-IB\_IRM ($d=0$) & \multicolumn{1}{c}{0.854(0.013)} & \multicolumn{1}{c}{0.863(0.018)} & \multicolumn{1}{c}{0.851(0.014)} & \multicolumn{1}{c}{0.843(0.014)} & \multicolumn{1}{c}{0.828(0.011)} \\
      P-IB\_IRM ($d=4$) & \multicolumn{1}{c}{0.863(0.016)} & \multicolumn{1}{c}{\underline{0.869(0.012)}} & \multicolumn{1}{c}{0.852(0.025)} & \multicolumn{1}{c}{0.858(0.013)} & \multicolumn{1}{c}{0.853(0.021)} \\
      P-IB\_IRM ($d=6$) & \multicolumn{1}{c}{\underline{0.866(0.013)}} & \multicolumn{1}{c}{0.865(0.015)} & \multicolumn{1}{c}{0.843(0.030)} & \multicolumn{1}{c}{\underline{0.860(0.023)}} & \multicolumn{1}{c}{\underline{0.860(0.013)}} \\
      P-IB\_IRM ($d=10$) & \multicolumn{1}{c}{0.865(0.021)} & \multicolumn{1}{c}{0.855(0.023)} & \multicolumn{1}{c}{\underline{0.854(0.024)}} & \multicolumn{1}{c}{0.852(0.013)} & \multicolumn{1}{c}{0.856(0.024)} \\
      \midrule
      \multicolumn{6}{c}{Avg. Minority Group Accuracy} \\
      \midrule
      ERM & \multicolumn{1}{c}{0.864(0.022)} & \multicolumn{1}{c}{0.862(0.039)} & \multicolumn{1}{c}{0.877(0.031)} & \multicolumn{1}{c}{0.868(0.030)} & \multicolumn{1}{c}{0.830(0.032)} \\
      P-ERM ($d=0$) & \multicolumn{1}{c}{0.876(0.019)} & \multicolumn{1}{c}{0.871(0.014)} & \multicolumn{1}{c}{\textbf{0.881(0.027)}} & \multicolumn{1}{c}{0.862(0.029)} & \multicolumn{1}{c}{0.844(0.015)} \\
      P-ERM ($d=4$) & \multicolumn{1}{c}{0.876(0.014)} & \multicolumn{1}{c}{0.887(0.017)} & \multicolumn{1}{c}{0.879(0.020)} & \multicolumn{1}{c}{0.863(0.018)} & \multicolumn{1}{c}{0.865(0.024)} \\
      P-ERM ($d=6$) & \multicolumn{1}{c}{0.888(0.027)} & \multicolumn{1}{c}{0.869(0.025)} & \multicolumn{1}{c}{0.878(0.021)} & \multicolumn{1}{c}{0.868(0.023)} & \multicolumn{1}{c}{0.881(0.019)} \\
      P-ERM ($d=10$) & \multicolumn{1}{c}{0.871(0.030)} & \multicolumn{1}{c}{0.878(0.028)} & \multicolumn{1}{c}{0.860(0.020)} & \multicolumn{1}{c}{0.863(0.023)} & \multicolumn{1}{c}{0.863(0.022)} \\
      \midrule
      IRM & \multicolumn{1}{c}{0.860(0.048)} & \multicolumn{1}{c}{0.874(0.026)} & \multicolumn{1}{c}{0.868(0.025)} & \multicolumn{1}{c}{0.864(0.047)} & \multicolumn{1}{c}{0.826(0.033)} \\
      P-IRM ($d=0$) & \multicolumn{1}{c}{0.866(0.015)} & \multicolumn{1}{c}{0.871(0.020)} & \multicolumn{1}{c}{0.859(0.023)} & \multicolumn{1}{c}{0.845(0.021)} & \multicolumn{1}{c}{0.832(0.018)} \\
      P-IRM ($d=4$) & \multicolumn{1}{c}{0.873(0.019)} & \multicolumn{1}{c}{0.880(0.014)} & \multicolumn{1}{c}{0.859(0.027)} & \multicolumn{1}{c}{0.864(0.016)} & \multicolumn{1}{c}{0.865(0.020)} \\
      P-IRM ($d=6$) & \multicolumn{1}{c}{0.880(0.023)} & \multicolumn{1}{c}{\textbf{0.882(0.018)}} & \multicolumn{1}{c}{0.850(0.041)} & \multicolumn{1}{c}{0.866(0.027)} & \multicolumn{1}{c}{0.871(0.021)} \\
      P-IRM ($d=10$) & \multicolumn{1}{c}{\textbf{0.888(0.020)}} & \multicolumn{1}{c}{0.857(0.030)} & \multicolumn{1}{c}{0.867(0.021)} & \multicolumn{1}{c}{0.866(0.014)} & \multicolumn{1}{c}{0.860(0.032)} \\
      \midrule
      IB\_IRM & 0.860(0.048) & 0.866(0.015) & 0.873(0.019) & \textbf{0.880(0.023)} & \textbf{0.888(0.020)} \\
      P-IB\_IRM ($d=0$) & \multicolumn{1}{c}{0.866(0.015)} & \multicolumn{1}{c}{0.871(0.020)} & \multicolumn{1}{c}{0.859(0.023)} & \multicolumn{1}{c}{0.845(0.021)} & \multicolumn{1}{c}{0.832(0.018)} \\
      P-IB\_IRM ($d=4$) & \multicolumn{1}{c}{0.873(0.019)} & \multicolumn{1}{c}{0.880(0.014)} & \multicolumn{1}{c}{0.859(0.027)} & \multicolumn{1}{c}{0.864(0.016)} & \multicolumn{1}{c}{0.865(0.020)} \\
      P-IB\_IRM ($d=6$) & \multicolumn{1}{c}{0.880(0.023)} & \multicolumn{1}{c}{0.882(0.018)} & \multicolumn{1}{c}{0.850(0.041)} & \multicolumn{1}{c}{0.866(0.027)} & \multicolumn{1}{c}{0.871(0.021)} \\
      P-IB\_IRM ($d=10$) & \multicolumn{1}{c}{0.888(0.020)} & \multicolumn{1}{c}{0.857(0.030)} & \multicolumn{1}{c}{0.867(0.021)} & \multicolumn{1}{c}{0.866(0.014)} & \multicolumn{1}{c}{0.860(0.032)} \\
      \midrule
      \multicolumn{6}{c}{Worst Group Accuracy} \\
      \midrule
      ERM & \multicolumn{1}{c}{0.825(0.032)} & \multicolumn{1}{c}{0.835(0.057)} & \multicolumn{1}{c}{0.830(0.036)} & \multicolumn{1}{c}{0.829(0.034)} & \multicolumn{1}{c}{0.805(0.031)} \\
      P-ERM ($d=0$) & 0.842(0.033) & 0.844(0.023) & 0.849(0.034) & 0.841(0.028) & 0.833(0.027) \\
      P-ERM ($d=4$) & \multicolumn{1}{c}{0.841(0.018)} & \multicolumn{1}{c}{0.859(0.018)} & \multicolumn{1}{c}{\textbf{0.853(0.019)}} & \multicolumn{1}{c}{0.844(0.039)} & \multicolumn{1}{c}{0.842(0.043)} \\
      P-ERM ($d=6$) & \multicolumn{1}{c}{0.839(0.023)} & \multicolumn{1}{c}{0.854(0.027)} & \multicolumn{1}{c}{0.850(0.022)} & \multicolumn{1}{c}{0.838(0.032)} & \multicolumn{1}{c}{0.854(0.019)} \\
      P-ERM ($d=10$) & 0.839(0.028) & 0.826(0.064) & 0.820(0.041) & 0.838(0.020) & 0.848(0.027) \\
      \midrule
      IRM & \multicolumn{1}{c}{0.826(0.064)} & \multicolumn{1}{c}{0.829(0.047)} & \multicolumn{1}{c}{0.811(0.028)} & \multicolumn{1}{c}{0.826(0.040)} & \multicolumn{1}{c}{0.797(0.034)} \\
      P-IRM ($d=0$) & \multicolumn{1}{c}{0.820(0.041)} & \multicolumn{1}{c}{0.834(0.034)} & \multicolumn{1}{c}{0.834(0.046)} & \multicolumn{1}{c}{0.821(0.025)} & \multicolumn{1}{c}{0.819(0.032)} \\
      P-IRM ($d=4$) & \multicolumn{1}{c}{0.838(0.020)} & \multicolumn{1}{c}{\textbf{0.853(0.033)}} & \multicolumn{1}{c}{0.838(0.033)} & \multicolumn{1}{c}{0.840(0.020)} & \multicolumn{1}{c}{0.832(0.043)} \\
      P-IRM ($d=6$) & \multicolumn{1}{c}{\textbf{0.848(0.027)}} & \multicolumn{1}{c}{0.835(0.038)} & \multicolumn{1}{c}{0.829(0.032)} & \multicolumn{1}{c}{\textbf{0.852(0.027)}} & \multicolumn{1}{c}{\textbf{0.849(0.012)}} \\
      P-IRM ($d=10$) & \multicolumn{1}{c}{0.836(0.039)} & \multicolumn{1}{c}{0.842(0.037)} & \multicolumn{1}{c}{0.840(0.043)} & \multicolumn{1}{c}{0.821(0.035)} & \multicolumn{1}{c}{0.848(0.036)} \\
      \midrule
      IB\_IRM & \multicolumn{1}{c}{0.826(0.064)} & \multicolumn{1}{c}{0.829(0.047)} & \multicolumn{1}{c}{0.811(0.028)} & \multicolumn{1}{c}{0.826(0.040)} & \multicolumn{1}{c}{0.797(0.034)} \\
      P-IB\_IRM ($d=0$) & \multicolumn{1}{c}{0.820(0.041)} & \multicolumn{1}{c}{0.834(0.034)} & \multicolumn{1}{c}{0.834(0.046)} & \multicolumn{1}{c}{0.821(0.025)} & \multicolumn{1}{c}{0.819(0.032)} \\
      P-IB\_IRM ($d=4$) & \multicolumn{1}{c}{0.838(0.020)} & \multicolumn{1}{c}{0.853(0.033)} & \multicolumn{1}{c}{0.838(0.033)} & \multicolumn{1}{c}{0.840(0.020)} & \multicolumn{1}{c}{0.832(0.043)} \\
      P-IB\_IRM ($d=6$) & \multicolumn{1}{c}{0.848(0.027)} & \multicolumn{1}{c}{0.835(0.038)} & \multicolumn{1}{c}{0.829(0.032)} & \multicolumn{1}{c}{0.852(0.027)} & \multicolumn{1}{c}{0.849(0.012)} \\
      P-IB\_IRM ($d=10$) & 0.836(0.039) & 0.842(0.037) & 0.840(0.043) & 0.821(0.035) & 0.848(0.036) \\
      \bottomrule
      \end{tabular}%
      \vspace{6pt}
    \caption{\textbf{Subpopulation shifts in MetaShift dataset}: The testing environments are observed during training, but differ in proportions. Results of models under the existence of minority environments in the training data. Here, the percentages of minority environments to the majority environments are $p \in \{50, 25, 12, 6, 1\}$. The lower the percentage the more challenging the training setting is. For P-x models, \textbf{\textit{d}} indicates the number of imported nodes at each partition. \textit{Underlined: for best among the same model, bold: best over all}.}    
    \label{tab:apx_subpopulation_all}%
  \end{table*}%


==> tables/non_optimal_dg_apx.tex <==
  % Table generated by Excel2LaTeX from sheet 'non-optimal_G_0'
  \begin{table*}[!ht]
    \centering
    
      \begin{tabular}{rlllll}
      \toprule
          &     & fence & shelf & floor & woman \\
      \midrule
      \multicolumn{1}{l}{Model} &     & s = 5.7 & s = 9.3 & s = 17.8 & s = 27.4 \\
      \midrule
      \multicolumn{1}{l}{P-ERM} & optimal partition & \textbf{0.714(0.020)} & \textbf{0.821(0.035)} & \textbf{0.777(0.030)} & \textbf{0.763(0.037)} \\
          & non-optimal  & 0.698(0.048) & 0.675(0.070) & 0.665(0.053) & 0.694(0.039) \\
      \midrule
      \multicolumn{1}{l}{P-IRM} & optimal partition & \textbf{0.721(0.041)} & \textbf{0.786(0.021)} & \textbf{0.741(0.035)} & \textbf{0.775(0.031)} \\
          & non-optimal  & 0.685(0.023) & 0.698(0.073) & 0.676(0.060) & 0.697(0.023) \\
      \midrule
      \multicolumn{1}{l}{P-IB\_IRM} & optimal partition & \textbf{0.713(0.038)} & \textbf{0.776(0.060)} & \textbf{0.736(0.039)} & \textbf{0.769(0.036)} \\
          & non-optimal  & 0.680(0.036) & 0.678(0.056) & 0.666(0.044) & 0.695(0.054) \\
      \bottomrule
      \end{tabular}%
      \vspace{6pt}
      \caption{Domain generalization experiment with non-optimal partitioning}
    \label{tab:nonoptimal_dg}%
  \end{table*}%

